Calibrating LLMs for Text-to-SQL Parsing by Leveraging Sub-clause Frequencies

While large language models (LLMs) achieve strong performance on text-to-SQL parsing, they sometimes exhibit unexpected failures in which they are confidently incorrect. Building trustworthy text-to-SQL systems thus requires eliciting reliable uncertainty measures from the LLM. In this paper, we study the problem of providing a calibrated confidence score that conveys the likelihood of an output query being correct. Our work is the first to establish a benchmark for post-hoc calibration of LLM-based text-to-SQL parsing. In particular, we show that Platt scaling, a canonical method for calibration, provides substantial improvements over directly using raw model output probabilities as confidence scores. Furthermore, we propose a method for text-to-SQL calibration that leverages the structured nature of SQL queries to provide more granular signals of correctness, named "sub-clause frequency" (SCF) scores. Using multivariate Platt scaling (MPS), our extension of the canonical Platt scaling technique, we combine individual SCF scores into an overall accurate and calibrated score. Empirical evaluation on two popular text-to-SQL datasets shows that our approach of combining MPS and SCF yields further improvements in calibration and the related task of error detection over traditional Platt scaling.

==> figures/cal_errors.tex <==
\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/images/ece.png}
    \includegraphics[width=1.0\textwidth]{figures/images/ace.png}
    \caption{For each combination of dataset and model, we aggregate the top and bottom 1\%, 5\%, 10\% of samples, ordered by the difference ($\Delta$) in the calibrated probability ouputted by Platt scaling (PS) and multiplicative Platt scaling (MPS) to summarize how adding features derived from parsing additional samples affects calibration. In addition, we report proportion of outputs in each quantile that are actually correct. Marker sizes on the scatter plot are sized according to the relative size of the bin.}
    \label{fig:ece}
\end{figure*}

==> figures/roc.tex <==
\begin{figure*}[htbp!]
    \centering
    % \includegraphics[width=1.0\textwidth]{figures/images/roc.png}
    \includegraphics[width=0.6\textwidth]{figures/images/roc_2x2.png}
    \caption{For each combination of dataset and model, we plot ROC curves for the problem of error detection using probabilities generated by (baseline) Platt scaling and (ours) multivariate Platt scaling.}
    \label{fig:roc}
\end{figure*}

==> tables/additional_analysis/calibration+auc_beam.tex <==
\begin{table*}[ht!]
\centering
\begin{tabular}{c c l c c c c}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Method} 
& \textbf{Brier} ($\downarrow$) & \textbf{ECE} ($\downarrow$) & \textbf{ACE} ($\downarrow$) & \textbf{AUC} ($\uparrow$) \\ 
\toprule

\multirow{6}{*}{SPIDER}

& \multirow{2}{*}{T5 3B}
&   PS          & 0.1626          & 0.0626          & 0.1102          & \textbf{0.8108} \\ 
& & MPS (beam)  & \textbf{0.1545} & \textbf{0.0261} & \textbf{0.0355} & 0.7873          \\

\cmidrule{2-7}

& \multirow{2}{*}{\textsc{Llama 3.1 8B Instruct}}
&   PS          & 0.1736          & 0.0449          & 0.0554          & 0.7260 \\ 
& & MPS (beam)  & \textbf{0.1705} & \textbf{0.0284} & \textbf{0.0344} & \textbf{0.7290} \\

\midrule

\multirow{6}{*}{BIRD}

& \multirow{2}{*}{\textsc{Llama 3.1 8B Instruct}}
&   PS          & 0.2121          & 0.0574          & 0.0737          & 0.6931 \\ 
& & MPS (beam)  & \textbf{0.1990} & \textbf{0.0385} & \textbf{0.0450} & \textbf{0.7195} \\

\cmidrule{2-7}

& \multirow{2}{*}{\textsc{Llama 3.1 70B Instruct}}
&   PS          & 0.2314          & 0.0499          & 0.0652          & 0.6669 \\ 
& & MPS (beam)  & \textbf{0.2211} & \textbf{0.0302} & \textbf{0.0375} & \textbf{0.6932} \\

\bottomrule
\end{tabular}
\caption{
    We report results for model outputs produced using only beam search. To derive sub-clause frequencies from the additional samples in the beam. We observe that \textbf{MPS} out performs \textbf{PS} w.r.t. calibration metrics in all settings. Our results suggest that using beam search, \textbf{MPS} provides improvements for calibration with minimal overhead (i.e., the additional computational workload of prompting the LLM for more samples). We note however that in terms of AUC of error detection, we observe mixed results for the SPIDER dataset, with \textbf{PS} outperforming \textbf{MPS} on outputs produced by \textsc{T5 3B}.
}
\label{tab:calibration+auc_beam}
\end{table*}




==> tables/additional_analysis/calibration+auc_nucleus.tex <==
\begin{table*}[ht!]
\centering
\begin{tabular}{c c l c c c c}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Method} 
& \textbf{Brier} ($\downarrow$) & \textbf{ECE} ($\downarrow$) & \textbf{ACE} ($\downarrow$) & \textbf{AUC} ($\uparrow$) \\ 
\toprule

\multirow{6}{*}{SPIDER}

& \multirow{2}{*}{\textsc{T5 3B}}
&   PS          & 0.1656 & 0.0622 & 0.0627 & 0.7200 \\ 
& & MPS (nucleus)  & 0.1638 & 0.0460 & 0.0539 & 0.7229          \\

\cmidrule{2-7}

& \multirow{2}{*}{\textsc{Llama 3.1 8B Instruct}}
&   PS          & 0.1740 & 0.0710 & 0.0818 & 0.7241 \\ 
& & MPS (nucleus)  & 0.1637 & 0.0292 & 0.0324 & 0.7449 \\

\midrule

\multirow{6}{*}{BIRD}

& \multirow{2}{*}{\textsc{Llama 3.1 8B Instruct}}
&   PS          & 0.2068 & 0.0501 & 0.1107 & 0.7373 \\ 
& & MPS (nucleus)  & 0.1908 & 0.0354 & 0.0310 & 0.7342 \\

\cmidrule{2-7}

& \multirow{2}{*}{\textsc{Llama 3.1 70B Instruct}}
&   PS          & 0.2274 & 0.0987 & 0.1005 & 0.7244 \\ 
& & MPS (nucleus)  & 0.2069 & 0.0314 & 0.0423 & 0.7416 \\

\bottomrule
\end{tabular}
\caption{
    We report results for model outputs produced using only nucleus sampling. To derive sub-clause frequencies, we use additional outputs produced from bean search only.
}
\label{tab:calibration+auc_nucleus}
\end{table*}




==> tables/additional_analysis/calibration_results_decode_type.tex <==
\begin{table*}[htbp!]
\centering
\begin{tabular}{c c c l c c c}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Decode Type} & \textbf{Method} & \textbf{Brier} & \textbf{ECE} & \textbf{ACE} \\ 
\toprule
\multirow{16}{*}{SPIDER}
& \multirow{8}{*}{T5 3B}
& \multirow{4}{*}{Nucleus}  
&     Token Probs.            & 0.1656           & 0.0622           & 0.0627          \\ 
& & & \quad + Beam            & \textbf{0.1564}  & \textbf{0.0240}  & 0.0307          \\ 
& & & \quad + Nucleus         & 0.1638           & 0.0460           & 0.0539          \\ 
& & & \quad + Nucleus + Beam  & 0.1566           & 0.0265           & \textbf{0.0253} \\
\cmidrule{3-7}
& & \multirow{4}{*}{Beam}
&     Token Probs.            & 0.1626           & 0.0626           & 0.1102          \\ 
& & & \quad + Beam            & \textbf{0.1545}  & 0.0261           & 0.0355          \\ 
& & & \quad + Nucleus         & 0.1615           & 0.0439           & 0.1067          \\ 
& & & \quad + Nucleus + Beam  & 0.1549           & \textbf{0.0256}  & \textbf{0250}   \\ 
\cmidrule{2-7}
& \multirow{8}{*}{\textsc{Llama 3.1 8B Instruct}}
& \multirow{4}{*}{Nucleus}
&     Token Probs.            & 0.1740           & 0.0710           & 0.0818          \\ 
& & & \quad + Beam            & 0.1694           & 0.0341           & 0.0324          \\ 
& & & \quad + Nucleus         & \textbf{0.1637}  & 0.0292           & 0.0324          \\ 
& & & \quad + Nucleus + Beam  & 0.1645           & \textbf{0.0274}  & \textbf{0.0274} \\
\cmidrule{3-7}
& & \multirow{4}{*}{Beam}
&     Token Probs.            & 0.1736           & 0.0449           & 0.0554          \\ 
& & & \quad + Beam            & 0.1705           & 0.0284           & 0.0344          \\ 
& & & \quad + Nucleus         & 0.1638           & \textbf{0.0253}  & \textbf{0.0270} \\ 
& & & \quad + Nucleus + Beam  & \textbf{0.1635}  & 0.0298           & \textbf{0.0270} \\ 
\midrule
\multirow{8}{*}{BIRD}
& \multirow{8}{*}{\textsc{Llama 3.1 8B Instruct}}
& \multirow{4}{*}{Nucleus}
& Token Probs.            & 0.2068           & 0.0501           & 0.1107          \\ 
& &   \quad + Beam            & 0.1920           & 0.0472           & 0.0472          \\ 
& & & \quad + Nucleus         & 0.1908           & \textbf{0.0354}  & \textbf{0.0310} \\ 
& & & \quad + Nucleus + Beam  & \textbf{0.1900}  & 0.0395           & 0.0383          \\
\cmidrule{3-7}
& &   \multirow{4}{*}{Beam}
&     Token Probs.            & 0.2121           & 0.0574           & 0.0737          \\ 
& & & \quad + Beam            & 0.1990           & 0.0385           & 0.0450          \\ 
& & & \quad + Nucleus         & 0.1963           & 0.0552           & 0.0581          \\ 
& & & \quad + Nucleus + Beam  & \textbf{0.1939}  & \textbf{0.0434}  & \textbf{0.0415} \\ 
\bottomrule
\end{tabular}
\caption{
Does decode type affect which method work best? Not really...
}
\label{tab:calibration_decode_type}
\end{table*}




\iffalse

SPIDER - T5
nucleus = 0.7352112676056338
beam = 0.7352112676056338


SPIDER - Llama 8B
nucleus = 0.7476635514018691
beam = 0.7377126654064272


BIRD - Llama 8B
nucleus = 0.3460231135282121
beam = 0.3564625850340136
nucleus + beam = 0.3585415259959487

\fi

==> tables/additional_analysis/compare_self_consistency.tex <==


\begin{table*}[ht!]
\centering
\begin{tabular}{lllcccc}
\toprule
\textbf{Method} & \textbf{Score Fn.} & \textbf{Brier} & \textbf{ECE} & \textbf{ACE} & \textbf{AUC} \\
\midrule
\multirow{2}{*}{Uncalibrated}
& Prob. & \textbf{0.1893} & \textbf{0.1632} & \textbf{0.1632} & \textbf{0.7200} \\
& SC & 0.1969 & 0.1706 & 0.1673 & 0.7097 \\
\midrule
\multirow{2}{*}{PS}
& Prob. & \textbf{0.1656} & 0.0623 & 0.0628 & \textbf{0.7200} \\
& SC & 0.1706 & \textbf{0.0620} & \textbf{0.0282} & 0.7097 \\
\midrule
\multirow{2}{*}{MPS (Beam)}
& Prob. & \textbf{0.1565} & \textbf{0.0241} & 0.0308 & \textbf{0.7804} \\
& SC & 0.1594 & 0.0280 & \textbf{0.0293} & 0.7696 \\
\midrule
\multirow{2}{*}{MPS (Nucleus)}
& Prob. & \textbf{0.1639} & \textbf{0.0460} & 0.0538 & \textbf{0.7229} \\
& SC & 0.1673 & 0.0462 & \textbf{0.0176} & 0.7139 \\
\midrule
\multirow{2}{*}{MPS (N + B)}
& Prob. & \textbf{0.1566} & \textbf{0.0264} & \textbf{0.0253} & \textbf{0.7785} \\
& SC & 0.1590 & 0.0273 & 0.0287 & 0.7707 \\
\bottomrule
\end{tabular}
\caption{
    Evaluating on \textsc{T5 3B} on SPIDER, we compare performance of our methods while varying the base scoring function (\textbf{Score Fn.}), choosing between either using model (log sum) token probabilities (\textbf{Prob.}) or using self-consistency (\textbf{SC}), which is derived by checking against the $k=10$ additional outputs produced from nucleus sampling. For methods, we evaluate the uncalibrated scoring functions (\textbf{Uncalibrated}), Platt scaling (\textbf{PS}), and multivariate Platt scaling (\textbf{MPS}) using SCF derived from nucleus sampling only (\textbf{Nucleus}), beam search only (\textbf{Beam}), and both (\textbf{N+B}). We observe little difference between using the two scoring functions.
}
\label{tab:compare_self_consistency_spider_t5}
\end{table*}


%%%%%

\begin{table*}[ht!]
\centering
\begin{tabular}{lllcccc}
\toprule
\textbf{Method} & \textbf{Score Fn.} & \textbf{Brier} & \textbf{ECE} & \textbf{ACE} & \textbf{AUC} \\
\midrule
\multirow{2}{*}{Uncalibrated}
& Prob. & 0.3576 & 0.4161 & 0.4147 & 0.7123 \\
& SC & \textbf{0.3428} & \textbf{0.3732} & \textbf{0.3793} & \textbf{0.7259} \\
\midrule
\multirow{2}{*}{PS}
& Prob. & 0.1726 & 0.0437 & 0.0449 & 0.7123 \\
& SC & \textbf{0.1679} & \textbf{0.0315} & \textbf{0.0315} & \textbf{0.7259} \\
\midrule
\multirow{2}{*}{MPS (Beam)}
& Prob. & 0.1687 & 0.0244 & \textbf{0.0230} & 0.7194 \\
& SC & \textbf{0.1650} & \textbf{0.0222} & 0.0291 & \textbf{0.7400} \\
\midrule
\multirow{2}{*}{MPS (Nucleus)}
& Prob. & 0.1625 & 0.0280 & 0.0360 & 0.7506 \\
& SC & \textbf{0.1612} & \textbf{0.0232} & \textbf{0.0312} & \textbf{0.7557} \\
\midrule
\multirow{2}{*}{MPS (N + B)}
& Prob. & 0.1626 & \textbf{0.0244} & 0.0260 & 0.7475 \\
& SC & \textbf{0.1611} & 0.0257 & \textbf{0.0232} & \textbf{0.7543} \\
\bottomrule
\end{tabular}
\caption{
    Evaluating on \textsc{Llama 3.1 8B Instruct} on SPIDER, we compare performance of our methods while varying the base scoring function (\textbf{Score Fn.}), choosing between either using model (log sum) token probabilities (\textbf{Prob.}) or using self-consistency (\textbf{SC}), which is derived by checking against the $k=10$ additional outputs produced from nucleus sampling. For methods, we evaluate the uncalibrated scoring functions (\textbf{Uncalibrated}), Platt scaling (\textbf{PS}), and multivariate Platt scaling (\textbf{MPS}) using SCF derived from nucleus sampling only (\textbf{Nucleus}), beam search only (\textbf{Beam}), and both (\textbf{N+B}). We observe little difference between using the two scoring functions.
}
\label{tab:compare_self_consistency_spider_llama_8b}
\end{table*}

%%%%%

\begin{table*}[ht!]
\centering
\begin{tabular}{lllcccc}
\toprule
\textbf{Method} & \textbf{Score Fn.} & \textbf{Brier} & \textbf{ECE} & \textbf{ACE} & \textbf{AUC} \\
\midrule
\multirow{2}{*}{Uncalibrated}
& Prob. & \textbf{0.2378} & \textbf{0.1722} & \textbf{0.1688} & \textbf{0.6913} \\
& SC & 0.2574 & 0.2150 & 0.2103 & 0.6577 \\
\midrule
\multirow{2}{*}{PS}
& Prob. & 0.2129 & 0.0556 & 0.0739 & \textbf{0.6913} \\
& SC & \textbf{0.2127} & \textbf{0.0432} & \textbf{0.0586} & 0.6577 \\
\midrule
\multirow{2}{*}{MPS (Beam)}
& Prob. & \textbf{0.1989} & \textbf{0.0425} & \textbf{0.0442} & \textbf{0.7213} \\
& SC & 0.1996 & 0.0428 & 0.0470 & 0.7204 \\
\midrule
\multirow{2}{*}{MPS (Nucleus)}
& Prob. & \textbf{0.1976} & \textbf{0.0574} & \textbf{0.0542} & \textbf{0.7307} \\
& SC & 0.1988 & 0.0588 & 0.0617 & 0.7243 \\
\midrule
\multirow{2}{*}{MPS (N + B)}
& Prob. & \textbf{0.1951} & 0.0418 & 0.0423 & \textbf{0.7347} \\
& SC & 0.1964 & \textbf{0.0408} & \textbf{0.0341} & 0.7301 \\
\bottomrule
\end{tabular}
\caption{
    Evaluating on \textsc{Llama 3.1 8B Instruct} on BIRD, we compare performance of our methods while varying the base scoring function (\textbf{Score Fn.}), choosing between either using model (log sum) token probabilities (\textbf{Prob.}) or using self-consistency (\textbf{SC}), which is derived by checking against the $k=10$ additional outputs produced from nucleus sampling. For methods, we evaluate the uncalibrated scoring functions (\textbf{Uncalibrated}), Platt scaling (\textbf{PS}), and multivariate Platt scaling (\textbf{MPS}) using SCF derived from nucleus sampling only (\textbf{Nucleus}), beam search only (\textbf{Beam}), and both (\textbf{N+B}). We observe little difference between using the two scoring functions.
}
\label{tab:compare_self_consistency_bird_llama_8b}
\end{table*}

%%%%%

\begin{table*}[ht!]
\centering
\begin{tabular}{lllcccc}
\toprule
\textbf{Method} & \textbf{Score Fn.} & \textbf{Brier} & \textbf{ECE} & \textbf{ACE} & \textbf{AUC} \\
\midrule
\multirow{2}{*}{Uncalibrated}
& Prob. & 0.2866 & 0.2343 & 0.2324 & 0.6650 \\
& SC & 0.3264 & 0.3128 & 0.3106 & 0.6798 \\
\midrule
\multirow{2}{*}{PS}
& Prob. & 0.2316 & 0.0549 & 0.0631 & 0.6650 \\
& SC & 0.2273 & 0.0512 & 0.0560 & 0.6798 \\
\midrule
\multirow{2}{*}{MPS (Beam)}
& Prob. & 0.2215 & 0.0384 & 0.0416 & 0.6921 \\
& SC & 0.2182 & 0.0278 & 0.0315 & 0.7047 \\
\midrule
\multirow{2}{*}{MPS (Nucleus)}
& Prob. & 0.2130 & 0.0290 & 0.0267 & 0.7203 \\
& SC & 0.2129 & 0.0304 & 0.0312 & 0.7213 \\
\midrule
\multirow{2}{*}{MPS (N + B)}
& Prob. & 0.1951 & 0.0418 & 0.0423 & 0.7347 \\
& SC & 0.2139 & 0.0224 & 0.0271 & 0.7183 \\
\bottomrule
\end{tabular}
\caption{
    Evaluating on \textsc{Llama 3.1 70B Instruct} on BIRD, we compare performance of our methods while varying the base scoring function (\textbf{Score Fn.}), choosing between either using model (log sum) token probabilities (\textbf{Prob.}) or using self-consistency (\textbf{SC}), which is derived by checking against the $k=10$ additional outputs produced from nucleus sampling. For methods, we evaluate the uncalibrated scoring functions (\textbf{Uncalibrated}), Platt scaling (\textbf{PS}), and multivariate Platt scaling (\textbf{MPS}) using SCF derived from nucleus sampling only (\textbf{Nucleus}), beam search only (\textbf{Beam}), and both (\textbf{N+B}). We observe little difference between using the two scoring functions.
}
\label{tab:compare_self_consistency_bird_llama_70b}
\end{table*}

==> tables/auc.tex <==
\begin{table*}[htbp!]
\centering
\begin{tabular}{c c l c}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Method} & \textbf{AUC}  \\ 
\toprule
\multirow{4}{*}{SPIDER}
& \multirow{2}{*}{\textsc{T5 3B}}                  & Token Probs.                                      & 0.7200  \\
&                                         & Token Probs. + Nucleus + Beam                     & 0.7785  \\ 
% &                                         & Token Probs. + Nucleus + Beam + Set Op. + Len.    & 0.7902  \\
\cmidrule{2-4}
& \multirow{2}{*}{\textsc{Llama 3.1 8B Instruct}}  & Token Probs.                                      & 0.7123  \\
&                                         & Token Probs. + Nucleus + Beam                     & 0.7475  \\ 
% &                                         & Token Probs. + Nucleus + Beam + Set Op. + Len.    & 0.7566  \\
\midrule
\multirow{2}{*}{BIRD}
& \multirow{2}{*}{\textsc{Llama 3.1 8B Instruct}}  & Token Probs.                                      & 0.6913  \\
&                                         & Token Probs. + Nucleus + Beam                     & 0.7353  \\ 
% &                                         & Token Probs. + Nucleus + Beam + Set Op. + Len.    & 0.7566  \\
\bottomrule
\end{tabular}
\caption{AUC for \textsc{T5 3B} and \textsc{Llama 3.1 8B Instruct}}
\label{tab:auc}
\end{table*}

==> tables/calibration_results.tex <==
\begin{table*}[htbp!]
\centering
\begin{tabular}{c c l c c c}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Method} & \textbf{Brier} & \textbf{ECE} & \textbf{ACE} \\ 
\toprule
% \hline
\multirow{6}{*}{SPIDER}
& \multirow{3}{*}{\textsc{T5 3B}}                    
&   Uncalibrated Token Probs.      & 0.1893           & 0.1632           & 0.1632          \\ 
& & Token Probs.                   & 0.1656           & 0.0623           & 0.0628          \\ 
& & Token Probs. + Nucleus + Beam  & \textbf{0.1566}  & \textbf{0.0264}  & \textbf{0.0253} \\
\cmidrule{2-6}
& \multirow{3}{*}{\textsc{Llama 3.1 8B Instruct}}
&   Uncalibrated Token Probs.      & 0.3576           & 0.4161           & 0.4147          \\ 
& & Token Probs.                   & 0.1726           & 0.0437           & 0.0449          \\ 
& & Token Probs. + Nucleus + Beam  & \textbf{0.1626}  & \textbf{0.0244}  & \textbf{0.0260} \\ 
\midrule
\multirow{3}{*}{BIRD}
% \multirow{6}{*}{BIRD}
% & \multirow{3}{*}{T5 3B}}
% &   Uncalibrated Token Probs.      & 0.1893           & 0.1632           & 0.1632          \\ 
% & & Token Probs.                   & 0.1656           & 0.0623           & 0.0628          \\ 
% & & Token Probs. + Nucleus + Beam  & \textbf{0.1566}  & \textbf{0.0264}  & \textbf{0.0253} \\ 
% \cmidrule{2-6}
& \multirow{3}{*}{\textsc{Llama 3.1 8B Instruct}}
&   Uncalibrated Token Probs.      & 0.2378           & 0.1722           & 0.1688          \\ 
& & Token Probs.                   & 0.2129           & 0.0556           & 0.0739          \\ 
& & Token Probs. + Nucleus + Beam  & \textbf{0.1950}  & \textbf{0.0418}  & \textbf{0.0423} \\ 
\bottomrule
\end{tabular}
\caption{We present Brier score, expected calibration error (ECE), and adaptive calibration Error (ACE) on the SPIDER and BIRD datasets. We calculate ECE and ACE using 10 bins. These metrics are calculated after applying Platt scaling to (baseline) token probabilities and (ours) token probabilities + parsed frequencies, which are derived from outputs obtained using nucleus sampling and beam search. For reference, we also include the performance of the token probabilities without calibration (i.e., applying Platt scaling).}
\label{tab:calibration}
\end{table*}

==> tables/model_accuracy.tex <==
\begin{table}[t]%[htbp!]
\centering
\begin{tabular}{c c c}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Accuracy} \\
\toprule

\multirow{2}{*}{SPIDER}
& \textsc{T5 3B}                & 73.52\% \\   
& \textsc{Llama 3.1 8B Instr.}  & 74.60\% \\       

\midrule

\multirow{2}{*}{BIRD}
& \textsc{Llama 3.1 8B Instr.}  & 35.85\% \\   
& \textsc{Llama 3.1 70B Instr.} & 53.35\% \\ 

\bottomrule
\end{tabular}
\caption{
We report the accuracy of each model on the corresponding dataset's test set.
}
\label{tab:model_acc}
\end{table}
